Large Language Models Can Self-Improve At Web Agent Tasks

Training models to act as agents that can effectively navigate and perform actions in a complex environment, such as a web browser, has typically been challenging due to lack of training data. Large language models (LLMs) have recently demonstrated some capability to navigate novel environments as agents in a zero-shot or few-shot fashion, purely guided by natural language instructions as prompts. Recent research has also demonstrated LLMs have the capability to exceed their base performance through self-improvement, i.e. fine-tuning on data generated by the model itself. In this work, we explore the extent to which LLMs can self-improve their performance as agents in long-horizon tasks in a complex environment using the WebArena benchmark. In WebArena, an agent must autonomously navigate and perform actions on web pages to achieve a specified objective. We explore fine-tuning on three distinct synthetic training data mixtures and achieve a 31\% improvement in task completion rate over the base model on the WebArena benchmark through a self-improvement procedure. We additionally contribute novel evaluation metrics for assessing the performance, robustness, capabilities, and quality of trajectories of our fine-tuned agent models to a greater degree than simple, aggregate-level benchmark scores currently used to measure self-improvement.

==> math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{color}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{bbm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
%\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
%\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\digit}[1]{\vcenter{\hbox{\includegraphics[height=10pt]{#1}}}}
\newcommand{\X}{\mathcal{X} }
\newcommand{\Sym}{\mathcal{S} }
\newcommand{\G}{\mathbf{G} }
\newcommand{\W}{\mathbf{W} }

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\s}[1]{\sout{#1}}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/Z-NeurIPSChecklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction (Section \ref{sec:introduction}) both introduce the claims and the scope of claims which are justified by the Sections \ref{sec:experiments} and \ref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{}
    \item[] Justification: Yes, we discuss this in a dedicated Limitations section in Section \ref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: The procedure and algorithms for data collection and generation are detailed in Section \ref{sec:data} and experiments are detailed in Section \ref{sec:experiments}. Detailed configuration and parameters for reproducibility can be found in Appendices \ref{sec:appendix_training_and_inference_details} and \ref{sec:appendix_prompts} and code/data is available in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer:  \answerYes{}
    \item[] Justification: Code and data is available in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Detailed configuration and parameters for reproducibility can be found in Appendices \ref{sec:appendix_training_and_inference_details} and \ref{sec:appendix_prompts} and code/data is available in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: We report a single evaluation run on the WebArena benchmark for all experiments, which is consistent with how results are reported in the WebArena paper in \cite{webarena}. Error bars are not reported because it would be too computationally expensive. The WebArena benchmark is an extremely resource-intensive benchmark requiring large models (we use a 72B parameter model) and requiring back-and-forth interaction between an LLM agent and a Chromium web browser which introduces a high amount of latency during evaluation (\textasciitilde 4-8 days per evaluation). Parallelization between experiments is also not easily possible due to the stateful nature of the environment. As stated by checklist instructions: \textit{it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive")}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Compute resources are detailed in Appendix \ref{sec:appendix_resources}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The research in this paper conforms, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: We discuss broader impacts in a dedicated section, Section \ref{sec:limitations}. We do not believe there to be significant broader impact concerns from this work, however, we note that self-distillation and self-improvement techniques can further reinforce incorrect behaviors and biases a model may already have through pre-training in Section \ref{sec:limitations}. All experiments were performed in the WebArena benchmark environment, which simulates websites in isolated Docker containers, ensuring our agent does not interfere with real, public websites during experimentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not believe this paper poses such risks. All experiments were performed in the WebArena benchmark environment, which simulates websites in isolated Docker containers, ensuring our agent does not interfere with real, public websites during experimentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: License information and citations for software, model, and data resources used are detailed in Appendix \ref{sec:appendix_resources} and cited throughout the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We release our code/data in the supplementary materials and detailed configuration and parameters for reproducibility can be found in Appendices \ref{sec:appendix_training_and_inference_details} and \ref{sec:appendix_prompts}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/appendices/F-CapabilitiesRaw.tex <==
{
\scriptsize

\textbf{Capability \#1:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What are the top-\texttt{\tiny \{\{n\}\}} best-selling product in \texttt{\tiny \{\{year\}\}}
\end{itemize}
\textbf{Capability \#2:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the the number of reviews that our store received by far that mention term ``\texttt{\tiny \{\{term\}\}}''
\end{itemize}
\textbf{Capability \#3:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What brands appear most frequently among the top search terms?
   \item List the top \texttt{\tiny \{\{n\}\}} search terms in my store
\end{itemize}
\textbf{Capability \#4:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Telll me the grand total of invoice \texttt{\tiny \{\{id\}\}}.
\end{itemize}
\textbf{Capability \#5:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Presents the monthly count of successful orders \texttt{\tiny \{\{period\}\}} in MM:COUNT format
\end{itemize}
\textbf{Capability \#6:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What's the total number of items sold in the most recent \texttt{\tiny \{\{k\}\}} orders?
\end{itemize}
\textbf{Capability \#7:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show all customers
\end{itemize}
\textbf{Capability \#8:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Give me the \texttt{\tiny \{\{Attribute\}\}} of the products that have \texttt{\tiny \{\{N\}\}} units left
\end{itemize}
\textbf{Capability \#9:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Get the total payment amount of the last \texttt{\tiny \{\{N\}\}} \texttt{\tiny \{\{status\}\}} orders
\end{itemize}
\textbf{Capability \#10:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Find the customer name and email with phone number \texttt{\tiny \{\{PhoneNum\}\}}
\end{itemize}
\textbf{Capability \#11:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the \texttt{\tiny \{\{attribute\}\}} of the customer who has the most cancellations in the history
   \item Which customer has completed the \texttt{\tiny \{\{quantifier\}\}} number of orders in the entire history?
   \item Show me the \texttt{\tiny \{\{information\}\}} of the customer who is the most unhappy with \texttt{\tiny \{\{product\}\}}
\end{itemize}
\textbf{Capability \#12:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How many reviews our shop received \texttt{\tiny \{\{time\}\}}?
   \item What is the total count of \texttt{\tiny \{\{status\}\}} reviews amongst all the reviews?
\end{itemize}
\textbf{Capability \#13:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Preview the \texttt{\tiny \{\{name\}\}} theme for my shop
\end{itemize}
\textbf{Capability \#14:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Mark all \texttt{\tiny \{\{brand\}\}} shirts on sale
\end{itemize}
\textbf{Capability \#15:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Disable \texttt{\tiny \{\{product\}\}} from the site, they are facing some quality issues.
\end{itemize}
\textbf{Capability \#16:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item \texttt{\tiny \{\{action\}\}} the price of \texttt{\tiny \{\{config\}\}} by \texttt{\tiny \{\{amount\}\}}
   \item \texttt{\tiny \{\{action\}\}} the price of this product by \texttt{\tiny \{\{amount\}\}}
\end{itemize}
\textbf{Capability \#17:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Update the description of \texttt{\tiny \{\{product\}\}} to highlight the real user positive reviews by quoting the comments
\end{itemize}
\textbf{Capability \#18:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Cancel order \texttt{\tiny \{\{id\}\}}
\end{itemize}
\textbf{Capability \#19:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Change the page title of ``\texttt{\tiny \{\{old-heading\}\}}'' page on my site to ``\texttt{\tiny \{\{heading\}\}}''.
\end{itemize}
\textbf{Capability \#20:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Notify \texttt{\tiny \{\{name\}\}} in their most recent pending order with message ``\texttt{\tiny \{\{message\}\}}''
\end{itemize}
\textbf{Capability \#21:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Update order \#\texttt{\tiny \{\{order\}\}} with the \texttt{\tiny \{\{service\}\}} tracking number \texttt{\tiny \{\{tracking\}\}}
\end{itemize}
\textbf{Capability \#22:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Make all \texttt{\tiny \{\{product\}\}} as out of stock
\end{itemize}
\textbf{Capability \#23:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Modify the address of order \#\texttt{\tiny \{\{order\_id\}\}} to \texttt{\tiny \{\{address\}\}}
\end{itemize}
\textbf{Capability \#24:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Add new \texttt{\tiny \{\{option\}\}} \texttt{\tiny \{\{value\}\}} to \texttt{\tiny \{\{base\_setting\}\}} of \texttt{\tiny \{\{product\}\}}
\end{itemize}
\textbf{Capability \#25:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Lookup orders that are \texttt{\tiny \{\{status\}\}}
   \item Get the \texttt{\tiny \{\{attribute\}\}} of the \texttt{\tiny \{\{status\}\}} order
\end{itemize}
\textbf{Capability \#26:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Add a simple product named \texttt{\tiny \{\{product\}\}} with \texttt{\tiny \{\{stock\}\}} in stock, available in size \texttt{\tiny \{\{size\}\}} and color \texttt{\tiny \{\{color\}\}}, priced at \$\texttt{\tiny \{\{price\}\}}
\end{itemize}
\textbf{Capability \#27:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Draft a new marketing price rule for \texttt{\tiny \{\{topic\}\}} that offers \texttt{\tiny \{\{rule\}\}} for all customers
\end{itemize}
\textbf{Capability \#28:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Today is 3/15/2023, generate a \texttt{\tiny \{\{report\}\}} \texttt{\tiny \{\{time\_span\}\}}
   \item Create a \texttt{\tiny \{\{type\}\}} report from \texttt{\tiny \{\{start\_date\}\}} to \texttt{\tiny \{\{end\_date\}\}}
\end{itemize}
\textbf{Capability \#29:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item We've received \texttt{\tiny \{\{quantity\}\}}, update the inventory.
\end{itemize}
\textbf{Capability \#30:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Approve the positive reviews to display in our store.
\end{itemize}
\textbf{Capability \#31:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Delete all \texttt{\tiny \{\{review\_type\}\}}
\end{itemize}
\textbf{Capability \#32:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the full address of all \texttt{\tiny \{\{airport\_type\}\}} that are within a driving distance of \texttt{\tiny \{\{radius\}\}} to \texttt{\tiny \{\{start\}\}}
\end{itemize}
\textbf{Capability \#33:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the \texttt{\tiny \{\{information\}\}} of \texttt{\tiny \{\{location\}\}}
   \item I will arrive \texttt{\tiny \{\{place\}\}} soon. Provide the name of a \texttt{\tiny \{\{target1\}\}} in the vicinity, if available. Then, tell me the \texttt{\tiny \{\{information\}\}} to \texttt{\tiny \{\{target2\}\}} from the hotel.
\end{itemize}
\textbf{Capability \#34:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the zip code of \texttt{\tiny \{\{place\}\}}?
\end{itemize}
\textbf{Capability \#35:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Given the following locations, \texttt{\tiny \{\{place\_list\}\}}, what would be the optimal route to travel through them all in order to minimize total travel time? Please note the journey begins at the first place listed.
\end{itemize}
\textbf{Capability \#36:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Which US states border \texttt{\tiny \{\{state\}\}}?
\end{itemize}
\textbf{Capability \#37:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Where is the nearest \texttt{\tiny \{\{places\}\}} to \texttt{\tiny \{\{start\}\}}, and what is the walking distance to it?
   \item Find the walkway to the closest \texttt{\tiny \{\{store\}\}} from \texttt{\tiny \{\{location\}\}}.
   \item How long does it take to walk from \texttt{\tiny \{\{start\}\}} to \texttt{\tiny \{\{end\}\}}?
   \item Tell me the closest \texttt{\tiny \{\{place1\}\}}(s) to \texttt{\tiny \{\{place2\}\}}
\end{itemize}
\textbf{Capability \#38:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item From my stay at \texttt{\tiny \{\{hotel\}\}}, what's the estimated driving time to reach \texttt{\tiny \{\{place\}\}}?
   \item What is the minimum travel time by car from \texttt{\tiny \{\{location1\}\}} to \texttt{\tiny \{\{location2\}\}}?
   \item What is the duration required to first walk from \texttt{\tiny \{\{place\_A\}\}} to \texttt{\tiny \{\{place\_B\}\}}, and then drive to \texttt{\tiny \{\{place\_C\}\}}?
   \item Show me the walking distance from nearby hotels to \texttt{\tiny \{\{location\}\}} that take at most \texttt{\tiny \{\{n\}\}} minutes?
   \item What is the estimated driving time between \texttt{\tiny \{\{city1\}\}} and \texttt{\tiny \{\{city2\}\}}?
\end{itemize}
\textbf{Capability \#39:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item From my stay at \texttt{\tiny \{\{hotel\}\}}, what's the estimated driving time to reach \texttt{\tiny \{\{place\}\}}?
   \item What is the estimated driving time between \texttt{\tiny \{\{city1\}\}} and \texttt{\tiny \{\{city2\}\}}?
   \item I am at CMU Pittsburgh, how long it takes to drive to the nearest \texttt{\tiny \{\{location\}\}}
   \item Check if the \texttt{\tiny \{\{place\}\}} in pittsburgh can be reached in one hour by car from \texttt{\tiny \{\{location\}\}}
\end{itemize}
\textbf{Capability \#40:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Find the \texttt{\tiny \{\{space\}\}} around \texttt{\tiny \{\{location\}\}}
   \item Find the walkway to the closest \texttt{\tiny \{\{store\}\}} from \texttt{\tiny \{\{location\}\}}.
   \item Tell me the closest \texttt{\tiny \{\{place1\}\}}(s) to \texttt{\tiny \{\{place2\}\}}
   \item Where is the nearest \texttt{\tiny \{\{location\}\}} from \texttt{\tiny \{\{location2\}\}} \texttt{\tiny \{\{condition\}\}}
\end{itemize}
\textbf{Capability \#41:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the \texttt{\tiny \{\{information\}\}} of \texttt{\tiny \{\{location\}\}}
   \item Tell me the coordinates of \texttt{\tiny \{\{location\}\}} in DD format
\end{itemize}
\textbf{Capability \#42:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How much time does it take from Pittsburgh to Philadelphia by car?
\end{itemize}
\textbf{Capability \#43:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show the route from SCS CMU in Pittsburgh to the location where the Declaration of Independence and Constitution were signed
\end{itemize}
\textbf{Capability \#44:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Pull up the description page of \texttt{\tiny \{\{location\}\}} on Map
   \item What is the \texttt{\tiny \{\{information\}\}} of \texttt{\tiny \{\{location\}\}}
\end{itemize}
\textbf{Capability \#45:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item I am arriving at Carnegie Mellon University. Find the nearby US Citizenship and Immigration Services and the walking distance to the nearest Social Security Administration from US Citizenship and Immigration Services
\end{itemize}
\textbf{Capability \#46:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item I am arriving at Pittsburgh Airport. Show me the name of a Hyatt hotel if there is any nearby. Tell me the names of supermarkets that are within 15mins driving from the hotel
\end{itemize}
\textbf{Capability \#47:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Measure distance between \texttt{\tiny \{\{location/address\_1\}\}} and \texttt{\tiny \{\{location/address\_2\}\}} by walking
   \item Get directions from \texttt{\tiny \{\{location/address\_1\}\}} to \texttt{\tiny \{\{location/address\_2\}\}} using \texttt{\tiny \{\{transportation\}\}} options.
\end{itemize}
\textbf{Capability \#48:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item List out reviewers, if exist, who mention about \texttt{\tiny \{\{description\}\}}
\end{itemize}
\textbf{Capability \#49:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Today is 6/12/2023. Tell me how many fulfilled orders I have \texttt{\tiny \{\{period\}\}}, and the total amount of money I spent.
\end{itemize}
\textbf{Capability \#50:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the status of my latest order and when will it arrive
\end{itemize}
\textbf{Capability \#51:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the date when I made my first purchase on this site?
\end{itemize}
\textbf{Capability \#52:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item I have jaw bruxism problem, show me something that could alleviate the problem.
\end{itemize}
\textbf{Capability \#53:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the price range for products from \texttt{\tiny \{\{brand\}\}}?
   \item What is the price range of \texttt{\tiny \{\{product\}\}} in the One Stop Market?
\end{itemize}
\textbf{Capability \#54:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How much I spent on \texttt{\tiny \{\{category\}\}} shopping during \texttt{\tiny \{\{time\}\}}
\end{itemize}
\textbf{Capability \#55:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the \texttt{\tiny \{\{option\}\}} configuration of the \texttt{\tiny \{\{product\}\}} I bought \texttt{\tiny \{\{time\}\}}
   \item I previously ordered some \texttt{\tiny \{\{product\}\}} \texttt{\tiny \{\{time\}\}} and later cancelled. Can you reorder it for me?
\end{itemize}
\textbf{Capability \#56:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item I have a lot of Nintendo Switch game cards now, help me find the best storage option to fit all \texttt{\tiny \{\{num\}\}} cards
\end{itemize}
\textbf{Capability \#57:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What are the main criticisms of this product? Please extract the relevant sentences.
\end{itemize}
\textbf{Capability \#58:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What do customers say about \texttt{\tiny \{\{product\_type\}\}} from \texttt{\tiny \{\{manufature\}\}}
\end{itemize}
\textbf{Capability \#59:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Buy the best rating product from ``\texttt{\tiny \{\{category\}\}}'' category with at least 5 reviews and the product is least expensive
   \item I am doing a market survey for one stop market, show me the most expensive product from \texttt{\tiny \{\{product\_category\}\}} category
   \item Buy the highest rated product from the \texttt{\tiny \{\{product\_category\}\}} category within a budget \texttt{\tiny \{\{dollar\_value\}\}}.
\end{itemize}
\textbf{Capability \#60:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Search for ``\texttt{\tiny \{\{keyword\}\}}''
\end{itemize}
\textbf{Capability \#61:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item List the full product names of slide slippers from Nike and tell me the price range of the available products
\end{itemize}
\textbf{Capability \#62:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Look up the most recent models of XBox controllers released between 2020-2021?
\end{itemize}
\textbf{Capability \#63:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show the least expensive \texttt{\tiny \{\{product\}\}} with a minimum storage capacity of \texttt{\tiny \{\{min\_storage\}\}}.
\end{itemize}
\textbf{Capability \#64:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show the most recent \texttt{\tiny \{\{status\}\}} order
   \item Get the order number of my most recent \texttt{\tiny \{\{status\}\}} order 
\end{itemize}
\textbf{Capability \#65:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Which number to call for the customer service?
\end{itemize}
\textbf{Capability \#66:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How much refund I should expect from my order canlled in \texttt{\tiny \{\{time\}\}}? I only kept the AC-DC Adapter and the shop told me that I cannot get the shipping fee back
\end{itemize}
\textbf{Capability \#67:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show me the ``\texttt{\tiny \{\{product\}\}}'' listings by \texttt{\tiny \{\{sorting\_order\}\}}.
\end{itemize}
\textbf{Capability \#68:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How much did I spend on shopping at One Stop Market \texttt{\tiny \{\{time\}\}}? They gave me a 20\% discount on the total amount for orders exceeding \$200 in cash
\end{itemize}
\textbf{Capability \#69:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me when I last ordered my \texttt{\tiny \{\{description\}\}}?
\end{itemize}
\textbf{Capability \#70:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item List products from \texttt{\tiny \{\{product\_category\}\}} category by \texttt{\tiny \{\{order\}\}} price
   \item Show me products under \$\texttt{\tiny \{\{price\}\}} in ``\texttt{\tiny \{\{product\_category\}\}}'' category
\end{itemize}
\textbf{Capability \#71:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show me the \texttt{\tiny \{\{info\}\}} for order number \texttt{\tiny \{\{order\_number\}\}}.
\end{itemize}
\textbf{Capability \#72:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item find discounted items.
\end{itemize}
\textbf{Capability \#73:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Summarize customer reviews for \texttt{\tiny \{\{product\}\}}.
\end{itemize}
\textbf{Capability \#74:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item List the customer names who thinks EYZUTAK phone cases are of good looking
   \item Who gave \texttt{\tiny \{\{stars\}\}} for phone cases from EYZUTAK
\end{itemize}
\textbf{Capability \#75:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What is the rating of \texttt{\tiny \{\{product\}\}}
\end{itemize}
\textbf{Capability \#76:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Add the product with the lowest per unit price from my open tabs to the shopping cart
\end{itemize}
\textbf{Capability \#77:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Add \texttt{\tiny \{\{product\}\}} to my wish list
   \item Add this product to my wishlist
   \item Add a \texttt{\tiny \{\{product\}\}} to my wish list.
\end{itemize}
\textbf{Capability \#78:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Subscribe to the newsletter of OneStopMarket
\end{itemize}
\textbf{Capability \#79:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item I recently moved, my address is \texttt{\tiny \{\{address\}\}}, update my information on OneStopShopping accordingly
   \item Change the delivery address for my most recent order to \texttt{\tiny \{\{address\}\}}.
\end{itemize}
\textbf{Capability \#80:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Rate my recent purchase of \texttt{\tiny \{\{product\}\}} with \texttt{\tiny \{\{num\_star\}\}} stars, using my nickname \texttt{\tiny \{\{nickname\}\}}?
\end{itemize}
\textbf{Capability \#81:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Fill the ``contact us'' form in the site for a refund on the \texttt{\tiny \{\{product\}\}} I bought, stating that it broke after just three days of use. Also, ensure to include the order number \#\texttt{\tiny \{\{order\_id\}\}} and the product SKU. Don't submit yet, I will check.
   \item Draft a refund message via their ``contact us'' form for the \texttt{\tiny \{\{product\}\}} I bought \texttt{\tiny \{\{time\}\}}. It broke after three days of use. The shop requires the order id, the reason and the amount to refund in the message. Don't submit yet
\end{itemize}
\textbf{Capability \#82:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Draft an email to the shop owner via their contact us function for a coupon as \texttt{\tiny \{\{reason\}\}}
\end{itemize}
\textbf{Capability \#83:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the count of comments that have received more downvotes than upvotes for the user who made the latest post on the \texttt{\tiny \{\{forum\}\}} forum.
\end{itemize}
\textbf{Capability \#84:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Among the top \texttt{\tiny \{\{number\}\}} post in ``\texttt{\tiny \{\{subreddit\}\}}'' forum, \texttt{\tiny \{\{description\}\}}
\end{itemize}
\textbf{Capability \#85:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Change my reddit bio to ``\texttt{\tiny \{\{content\}\}}''
\end{itemize}
\textbf{Capability \#86:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Reply to \texttt{\tiny \{\{position\_description\}\}} with my comment ``\texttt{\tiny \{\{content\_description\}\}}''
\end{itemize}
\textbf{Capability \#87:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Create a new forum named \texttt{\tiny \{\{name\}\}}, with a description of \texttt{\tiny \{\{description\}\}}, and include \texttt{\tiny \{\{sidebar\_list\}\}} in the sidebar?
\end{itemize}
\textbf{Capability \#88:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Open the thread of a trending post on the forum ``\texttt{\tiny \{\{subreddit\}\}}'' and subscribe.
   \item Upvote the newest post in \texttt{\tiny \{\{subreddit\}\}} subreddit
\end{itemize}
\textbf{Capability \#89:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Create a discussion post about ``\texttt{\tiny \{\{topic\}\}}'' in a relevant subreddit and ask users for their opinions with the simple prompt, ``your opinion''
   \item Find a subreddit focused on topics related to \texttt{\tiny \{\{topic\}\}}, and post my question, ``\texttt{\tiny \{\{question\}\}}'' there
   \item Post my question, ``\texttt{\tiny \{\{question\}\}}\ in a subreddit where I'm likely to get an answer
\end{itemize}
\textbf{Capability \#90:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Post a review of my recent reading ``\texttt{\tiny \{\{book\}\}}'' in the r/books with my comment ``\texttt{\tiny \{\{content\}\}}''.
\end{itemize}
\textbf{Capability \#91:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Re-post the image of \texttt{\tiny \{\{content\}\}} in this page to \texttt{\tiny \{\{subreddit\}\}} subreddit and note ``from /f/pics''
\end{itemize}
\textbf{Capability \#92:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Ask for advice about \texttt{\tiny \{\{issue\}\}} in a subreddit for relations
\end{itemize}
\textbf{Capability \#93:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Post in the most appropriate subreddit and ask for recommendations for \texttt{\tiny \{\{category\}\}} products within a budget of \texttt{\tiny \{\{price\}\}}
   \item Ask for product recommendations for \texttt{\tiny \{\{category\}\}} within a budget of \texttt{\tiny \{\{price\}\}} in \texttt{\tiny \{\{subreddit\}\}}
\end{itemize}
\textbf{Capability \#94:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Post a notice on a virtual meetup for \texttt{\tiny \{\{interest\}\}} enthusiasts on \texttt{\tiny \{\{date\}\}} in the \texttt{\tiny \{\{subreddit\}\}} subreddit
\end{itemize}
\textbf{Capability \#95:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Post in \texttt{\tiny \{\{subreddit\}\}} subreddit about what could diffusion model help the correpong field.
\end{itemize}
\textbf{Capability \#96:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Thumbs down the top \texttt{\tiny \{\{k\}\}} post ever in \texttt{\tiny \{\{subreddit\}\}}.
\end{itemize}
\textbf{Capability \#97:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Like all submissions created by \texttt{\tiny \{\{user\}\}} in subreddit \texttt{\tiny \{\{subreddit\}\}}
   \item DisLike all submissions created by \texttt{\tiny \{\{user\}\}} in subreddit \texttt{\tiny \{\{subreddit\}\}}
\end{itemize}
\textbf{Capability \#98:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Edit my post on \texttt{\tiny \{\{post\}\}} by adding a line to the body that says ``\texttt{\tiny \{\{content\}\}}''
\end{itemize}
\textbf{Capability \#99:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Check out my todos
\end{itemize}
\textbf{Capability \#100:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Check out the most recent open issues
\end{itemize}
\textbf{Capability \#101:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Checkout merge requests assigned to me
   \item Checkout merge requests requiring my review
\end{itemize}
\textbf{Capability \#102:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the full names of the repositories where I made contributions and they got \texttt{\tiny \{\{description\}\}} stars?
\end{itemize}
\textbf{Capability \#103:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Open my latest created issue that has \texttt{\tiny \{\{keyword\}\}} in its title to check if it is closed
   \item Open my latest updated issue that has keyword ``\texttt{\tiny \{\{keyword\}\}}'' in its title to check if it is closed
\end{itemize}
\textbf{Capability \#104:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item See all public projects
\end{itemize}
\textbf{Capability \#105:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Get me my RSS feed token
\end{itemize}
\textbf{Capability \#106:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show me the command to clone \texttt{\tiny \{\{repo\}\}} with SSH.
\end{itemize}
\textbf{Capability \#107:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item List all opened issues \texttt{\tiny \{\{description\}\}}
\end{itemize}
\textbf{Capability \#108:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Who else have access to my repo \texttt{\tiny \{\{repo\}\}}, show me their usernames
\end{itemize}
\textbf{Capability \#109:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Post ``\texttt{\tiny \{\{content\}\}}'' for the merge request related to \texttt{\tiny \{\{mr\}\}} in \texttt{\tiny \{\{repo\}\}} project
\end{itemize}
\textbf{Capability \#110:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Fork \texttt{\tiny \{\{repo\}\}}.
\end{itemize}
\textbf{Capability \#111:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Make the LICENSE of \texttt{\tiny \{\{repo\}\}} to MIT license.
\end{itemize}
\textbf{Capability \#112:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Go to the merge request on \texttt{\tiny \{\{topic\}\}} I have to review, find if the author of the merge request responded at the end, and reply ``Thank you'' if he did. Otherwise remind him with a simple @.
\end{itemize}
\textbf{Capability \#113:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Set my gitlab status as \texttt{\tiny \{\{status\}\}}.
\end{itemize}
\textbf{Capability \#114:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Update the project site's title to ``\texttt{\tiny \{\{title\}\}}''
\end{itemize}
\textbf{Capability \#115:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item set the homepage URL on my GitLab profile to \texttt{\tiny \{\{url\}\}}
\end{itemize}
\textbf{Capability \#116:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Set up a new, empty repository with the name \texttt{\tiny \{\{project\_name\}\}}?
   \item Create a private \texttt{\tiny \{\{template\}\}} repository called ``\texttt{\tiny \{\{project\_name\}\}}'' using the right template to speed up development.
\end{itemize}
\textbf{Capability \#117:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Invite \texttt{\tiny \{\{collaborator\_account\_list\}\}} as collaborator to \texttt{\tiny \{\{repo\}\}} repo
   \item Add the following users to repo \texttt{\tiny \{\{repo\}\}} as \texttt{\tiny \{\{role\}\}}: \texttt{\tiny \{\{user\_list\}\}}
\end{itemize}
\textbf{Capability \#118:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item \texttt{\tiny \{\{name\}\}} wants to check my dotfile configurations. Please invite him to the repo as a guest.
\end{itemize}
\textbf{Capability \#119:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Star the top \texttt{\tiny \{\{number\}\}} most stared repos in Gitlab
\end{itemize}
\textbf{Capability \#120:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Follow \texttt{\tiny \{\{account\_list\}\}} on Gitlab
\end{itemize}
\textbf{Capability \#121:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Create a milestone for the upcoming \texttt{\tiny \{\{event\}\}} starting on \texttt{\tiny \{\{start\_date\}\}} and ending on \texttt{\tiny \{\{end\_date\}\}}
\end{itemize}
\textbf{Capability \#122:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Create an issue \texttt{\tiny \{\{issue\}\}} in \texttt{\tiny \{\{repo\}\}}.
   \item Assign the issue regarding \texttt{\tiny \{\{issue\}\}} in \texttt{\tiny \{\{repo\}\}} to \texttt{\tiny \{\{account\}\}}.
   \item Create an issue in \texttt{\tiny \{\{repo\}\}} repo with title ``\texttt{\tiny \{\{issue\}\}}''. Assign the issue to \texttt{\tiny \{\{account\}\}}. Set due date to be \texttt{\tiny \{\{due\}\}}
\end{itemize}
\textbf{Capability \#123:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Submit a merge request for \texttt{\tiny \{\{source\_branch\}\}} branch to be merged into \texttt{\tiny \{\{target\_branch\}\}} branch, assign \texttt{\tiny \{\{reviewer\}\}} as the reviewer
\end{itemize}
\textbf{Capability \#124:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Open a new issue to discuss the implementation of \texttt{\tiny \{\{feature\}\}}
\end{itemize}
\textbf{Capability \#125:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Start a private project \texttt{\tiny \{\{project\_name\}\}} with \texttt{\tiny \{\{template\}\}} template and add \texttt{\tiny \{\{account\_list\}\}} as members
\end{itemize}
\textbf{Capability \#126:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item How many commits did \texttt{\tiny \{\{user\}\}} make on \texttt{\tiny \{\{date\}\}} in total?
   \item Tell me who has made the most contributions, in terms of number of commits, to the \texttt{\tiny \{\{repo\}\}} project
   \item Tell me the \texttt{\tiny \{\{attribute\}\}} of the contributor who has the most commits to branch \texttt{\tiny \{\{branch\_name\}\}}
   \item List the \texttt{\tiny \{\{attribute\}\}} of the top 3 contributors to \texttt{\tiny \{\{repo\}\}} repo, ranked by the number of commits?
\end{itemize}
\textbf{Capability \#127:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item create a new group ``\texttt{\tiny \{\{name\}\}}'' with members \texttt{\tiny \{\{members\}\}}
\end{itemize}
\textbf{Capability \#128:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Tell me the distance to drive from Carnegie Mellon University to the top computer science school in massachusetts
\end{itemize}
\textbf{Capability \#129:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item What's the closest national park to \texttt{\tiny \{\{city\}\}}? How long does it take to bike there?
\end{itemize}
\textbf{Capability \#130:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Find the page of \texttt{\tiny \{\{description\}\}} on the map.
\end{itemize}
\textbf{Capability \#131:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show me the way from \texttt{\tiny \{\{location\}\}} to the home stadium of \texttt{\tiny \{\{sport\_team\}\}} \texttt{\tiny \{\{time\}\}}
\end{itemize}
\textbf{Capability \#132:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Find a GitLab repository related to \texttt{\tiny \{\{topic\}\}} and make a Reddit post linking to it in a relevant subreddit
   \item create a repository named \texttt{\tiny \{\{name\}\}} that includes a README file with the links to the most active \texttt{\tiny \{\{num\}\}} DIY ideas on DIY subreddit?
   \item Make a folder named \texttt{\tiny \{\{directory\}\}} on the \texttt{\tiny \{\{gitlab\_repo\}\}} repo and include a file called urls.txt that consists of the links to the 5 most recent posts from \texttt{\tiny \{\{subreddit\}\}}.
\end{itemize}
\textbf{Capability \#133:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Promote \texttt{\tiny \{\{repo\}\}} to subreddit \texttt{\tiny \{\{subreddit\}\}} with the description from the repo itself.
\end{itemize}
\textbf{Capability \#134:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Create a repo named \texttt{\tiny \{\{name\}\}} with \texttt{\tiny \{\{topics\}\}} in a README file
\end{itemize}
\textbf{Capability \#135:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Gather the titles of \texttt{\tiny \{\{product\}\}} reviews with \texttt{\tiny \{\{rating\}\}} rating from OneStopShop, and post them in the games subreddit under the title ``real user feedback on \texttt{\tiny \{\{product\}\}}''
\end{itemize}
\textbf{Capability \#136:}
\begin{itemize}[noitemsep,leftmargin=*]
   \item Show me the route and driving time from \texttt{\tiny \{\{city1\}\}} to \texttt{\tiny \{\{city2\}\}}
\end{itemize}

}

